C programs for solving the time-dependent Gross-Pitaevskii equation in a fully anisotropic trap

We present C programming language versions of earlier published Fortran programs (Muruganandam and Adhikari, Comput. Phys. Commun. 180 (2009) 1888) for calculating both stationary and non-stationary solutions of the time-dependent Gross-Pitaevskii (GP) equation. The GP equation describes the properties of dilute Bose-Einstein condensates at ultra-cold temperatures. C versions of programs use the same algorithms as the Fortran ones, involving real- and imaginary-time propagation based on a split-step Crank-Nicolson method. In a one-space-variable form of the GP equation, we consider the one-dimensional, two-dimensional, circularly-symmetric, and the three-dimensional spherically-symmetric harmonic-oscillator traps. In the two-space-variable form, we consider the GP equation in two-dimensional anisotropic and three-dimensional axially-symmetric traps. The fully-anisotropic three-dimensional GP equation is also considered. In addition to these twelve programs, for six algorithms that involve two and three space variables, we have also developed threaded (OpenMP parallelized) programs, which allow numerical simulations to use all available CPU cores on a computer. All 18 programs are optimized and accompanied by makefiles for several popular C compilers. We present typical results for scalability of threaded codes and demonstrate almost linear speedup obtained with the new programs, allowing a decrease in execution times by an order of magnitude on modern multi-core computers.

==> GP-SCL-programs/makefile <==
# 
# GP-SCL codes are developed by:
# 
# Dusan Vudragovic, Ivana Vidanovic, Antun Balaz
# (Institute of Physics Belgrade, Serbia, http://www.scl.rs/)
# 
# Paulsamy Muruganandam
# (Bharathidasan University, Tamil Nadu, India)
# 
# Sadhan K. Adhikari
# (Sao Paulo State University, Brazil)
#    
# Public use and modification of this code are allowed provided that the
# following papers are cited:
# P. Muruganandam et al., Comput. Phys. Commun. 180 (2009) 1888;
# D. Vudragovic et al., Comput. Phys. Commun. 183 (2012) 2021.
# The authors would be grateful for all information and/or comments regarding
# the use of the code.
#

CC = gcc
CFLAGS = -O5
OMPFLAGS = -fopenmp
LIBS = -lm
OMPLIBS = -lpthread

ifeq ($(compiler), icc)
	CC = icc
	CFLAGS = -fast
	OMPFLAGS = -openmp
	LIBS = -lm
	OMPLIBS = -lpthread
endif

ifeq ($(compiler), xlc)
	CC = xlc
	CFLAGS = -O5 -q64
	OMPFLAGS = -qsmp=omp
	LIBS = -lm
	OMPLIBS = -qthreaded
endif

ifeq ($(compiler), pgcc)
	CC = pgcc
	CFLAGS = -fast
	OMPFLAGS = -mp
	LIBS = -lm
	OMPLIBS = -lpthread
endif

ifeq ($(compiler), suncc)
	CC = suncc
	CFLAGS = -O3 -fast
	OMPFLAGS = -xopenmp
	LIBS = -lm
	OMPLIBS = -lpthread
endif

SERIAL_TARGETS=imagtime1d imagtime2d imagtime3d \
               imagtimeaxial imagtimecir imagtimesph \
               realtime1d realtime2d realtime3d \
               realtimeaxial realtimecir realtimesph
SERIAL_OBJECTS=$(SERIAL_TARGETS:=.o)

OPENMP_TARGETS=imagtime2d-th imagtime3d-th imagtimeaxial-th \
               realtime2d-th realtime3d-th realtimeaxial-th
OPENMP_OBJECTS=$(OPENMP_TARGETS:=.o)

UTIL_TARGETS=diffint mem cfg
UTIL_OBJECTS=$(UTIL_TARGETS:=.o)

all: $(SERIAL_TARGETS) $(OPENMP_TARGETS)
	@rm -rf $(UTIL_OBJECTS)

serial: $(SERIAL_TARGETS)
	@rm -rf $(UTIL_OBJECTS)

openmp: $(OPENMP_TARGETS)
	@rm -rf $(UTIL_OBJECTS)

help: readme.txt
	less $^

$(SERIAL_TARGETS): % : $(UTIL_OBJECTS) %.o
	$(CC) $(CFLAGS) -o $@ $@.o $(UTIL_OBJECTS) $(LIBS)
	@rm -rf $@.o

$(OPENMP_TARGETS): % : $(UTIL_OBJECTS) %.o
	$(CC) $(CFLAGS) $(OMPFLAGS) -o $@ $@.o $(UTIL_OBJECTS) $(LIBS) $(OMPLIBS)
	@rm -rf $@.o

$(SERIAL_OBJECTS): %.o:
	$(CC) $(CFLAGS) -c src/$*/$*.c -o $@

$(OPENMP_OBJECTS): %.o:
	$(CC) $(CFLAGS) $(OMPFLAGS) -c src/$*/$*.c -o $@

$(UTIL_OBJECTS): %.o:
	$(CC) $(CFLAGS) -c src/util/$*.c -o $@

clean:
	@rm -rf $(SERIAL_TARGETS) $(OPENMP_TARGETS) \
           $(SERIAL_OBJECTS) $(OPENMP_OBJECTS) \
           $(UTIL_OBJECTS)

